Multi-Granularity Guided Fusion-in-Decoder

In Open-domain Question Answering (ODQA), it is essential to discern relevant contexts as evidence and avoid spurious ones among retrieved results. The model architecture that uses concatenated multiple contexts in the decoding phase, i.e., Fusion-in-Decoder, demonstrates promising performance but generates incorrect outputs from seemingly plausible contexts. To address this problem, we propose the Multi-Granularity guided Fusion-in-Decoder (MGFiD), discerning evidence across multiple levels of granularity. Based on multi-task learning, MGFiD harmonizes passage re-ranking with sentence classification. It aggregates evident sentences into an anchor vector that instructs the decoder. Additionally, it improves decoding efficiency by reusing the results of passage re-ranking for passage pruning. Through our experiments, MGFiD outperforms existing models on the Natural Questions (NQ) and TriviaQA (TQA) datasets, highlighting the benefits of its multi-granularity solution.

==> temp.tex <==
\section{Related Work} \label{sec:related_work}
\noindent
% \subsection{Open-domain Question Answering (ODQA)}\label{sec:related_ODQA}
% \textbf{Open-domain Question Answering (ODQA).}\label{sec:related_ODQA}
Retrieval-augmented generation(RAG) approach has become influential for knowledge-intensive tasks by combining advanced generative language models with information from vast external databases. \citet{nips/LewisPPPKGKLYR020/RAG} proposed to fetch a representation of relevant top-$k$ documents and generate an output token distribution for each context. \citet{icml/BorgeaudMHCRM0L22/RETRO, corr/abs-2302-00083/In-ContextRALM} proposed to dynamically pull retrieval results during the generation process to enhance the relevance of the information being integrated.
FiD uses a large key-value matrix concatenated after encoding each context~\cite{eacl/IzacardG21/FiD}. This framework has verified that the T5-decoder~\cite{JMLR/Raffel2020/T5} can effectively aggregate the evidence contained in multiple documents. Several studies have built on FiD's evidence aggregation capability: ~\citet{iclr/IzacardG21/FiD-KD, emnlp/LeeKLPMW22/YONO} performed knowledge distillation on a retriever with cross-attention scores obtained during the generation. ~\citet{nips/SachanRHDY21/EMDR2} proposed end-to-end training of FiD reader and retriever. On the other hand, ~\citet{iclr/YuIWXJSZZJ23/GenREAD, corr/abs-2310-14393/COMBO} enhanced the contexts with LLM-generated contexts. While improving the quality of input has been shown to improve ODQA performance, validating the reference is implicit since readers in these studies are only focused on generating answers. Given that the input contexts are not ground-truth, the reader may be vulnerable to noise, hence reading the given contexts with proper discernment is an emerging challenge to be addressed.

% \subsection{Evidential RAG}\label{sec:Multi-task}
% There have been studies that add learning modules that help FiD readers to be robust to the noise in search results and focus on the real evidence. One important study is how to utilize factual information contained in Knowledge Graphs (KGs). In the last layer of the FiD encoder, \citet{acl/Yu0F0WXRY022/KG-FiD} incorporates the textual semantic information in embeddings with the knowledge graph to perform re-ranking for the top $k$ contexts. They also improved efficiency by passing only the high-ranked contexts to the decoder. On the other hand, ~\citet{emnlp/Ju00Z022/GRAPE} extracts entity embeddings from the intermediate layer and combines embeddings with graph knowledge fused through GNN. While relational information from KG is trustful and helps avoid contradictions, it has a limited scope as it requires external data.
% Defining rationale labels without external knowledge and performing multi-task learning~\cite{emnlp/LakhotiaPGYMI21/FiD-Ex, sigir/HofstatterC0Z23/FiD-Light, acl/WangY023/RFiD} is one approach to empowering FiD with discernment of evidentiality.
\subsection{Evidence-based learning}\label{sec:}
Since FiD trained solely to generate the answer can fall back on spurious passages, several works incorporate multi-task learning to provide the model discrimination. \citet{emnlp/LakhotiaPGYMI21/FiD-Ex} proposed a special sentence marker token to enable the decoder to generate a marker corresponding to the grounds along with the answer. \citet{acl/WangY023/RFiD} introduced a binary classifier that can determine whether each passage is supported between the encoder and decoder. Furthermore, they proposed to append learnable embeddings that correspond to predictions, which can guide decoding. In most OpenQA settings where gold context annotation does not exist, the way these works define groundedness follows the narrow way used in the original work~\cite{emnlp/KarpukhinOMLWEC20/DPR}, \ie, whether the answer span is included. However, the inclusion of the answer span does not guarantee evidentiality and leads to sub-optimal results. ~\citet{naacl/Asai0H22/EvidentialityQA} pointed out this limitation and suggested a classifier for mining pseudo-evidentiality labels. However, they still require expensive annotations to train the classifier, and labeling with a partially trained model can be affected by the model's memorization.

\subsection{Decoding efficiency}\label{sec:related_efficiency}
Simply reducing the number of FiD input passages is not as optimal as reducing the decoder input alone~\cite{sigir/HofstatterC0Z23/FiD-Light}. Previous work has reduced the burden on the decoder by taking only necessary parts of the given information.
~\citet{sigir/HofstatterC0Z23/FiD-Light} reduce the length of each encoded query-passage pair to the first few vectors. By compressing the amount of information fed to the decoder, it can significantly improve inference efficiency while slightly reducing effectiveness.
\citet{acl/Yu0F0WXRY022/KG-FiD} incorporates the textual semantic information in embeddings of the last layer of the FiD encoder, with the knowledge graph to perform re-ranking for the top $k$ contexts. They improved efficiency by passing only the high-ranked contexts to the decoder.
